G-STAR: Group-Scaled Token Capacity for Deeply Compressed Autoregressive Generation

Discrete autoregressive models offer a scalable framework for image generation. However, they face a fundamental trade-off: long token sequences preserve representation quality but slow generation, while aggressive spatial compression reduces representation capacity. Based on product quantization, we show that, under a fixed nominal information budget, group size should scale quadratically with the per-axis spatial compression factor. Building on this principle, we propose GSTAR, a spatial--group co-scaling framework that enables \(32\times\) and even effective \(64\times\) compression while preserving strong reconstruction, understanding, and generation performance. Since larger groups introduce intra-group dependencies that must be modeled efficiently, we analyze their impact on inference latency and generation quality and introduce a semi-autoregressive decoder that combines parallel feature computation with lightweight causal modeling. With these designs, our highly compressed models perform competitively with leading models across five representative text-to-image benchmarks (GenEval, DPG-Bench, PRISM, LongText-Bench, and Qwen-Image-Bench). At \(1024\times1024\) resolution, our model delivers a \(20\times\) speedup over prior discrete autoregressive models, generating each image in 2.5 seconds on a single NVIDIA H200. Together, these results show that highly compressed discrete representations can enable high-quality autoregressive generation at low latency.

==> tables/group_scaling.tex <==
\begin{table}[t]
\centering
\small
\caption{Effects of group size with $K=16{,}384$.}
\label{tab:group_scaling}
\begin{tabular}{crrr}
\toprule
Group size $G$ & rFID $\downarrow$ & gFID $\downarrow$
& Linear probing (\%) $\uparrow$ \\
\midrule
1  & 2.0624 & \textbf{2.1057} & 81.45 \\
8  & 0.8525 & 6.3773        & 82.90 \\
16 & 0.5357 & 5.7388          & 84.15 \\
32 & \textbf{0.4325} & 17.05  & \textbf{84.55} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/group_scaling_t2i.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Text-to-image group-size ablation under the same
training settings. PRISM reports the combined score
on a 0--10 scale. All metrics are higher-is-better.}
\label{tab:group_scaling_t2i}
\begin{tabular}{crrr}
\toprule
Group size $G$ & GenEval $\uparrow$ & DPG-Bench $\uparrow$
& PRISM $\uparrow$ \\
\midrule
8  & 0.8060 & 82.49 & 5.30 \\
16 & 0.8386 & 82.48 & 5.46 \\
\bottomrule
\end{tabular}
\end{table}
